ELDA: Using Edges to Have an Edge on Semantic Segmentation Based UDA

Many unsupervised domain adaptation (UDA) methods have been proposed to bridge the domain gap by utilizing domain invariant information. Most approaches have chosen depth as such information and achieved remarkable success. Despite their effectiveness, using depth as domain invariant information in UDA tasks may lead to multiple issues, such as excessively high extraction costs and difficulties in achieving a reliable prediction quality. As a result, we introduce Edge Learning based Domain Adaptation (ELDA), a framework which incorporates edge information into its training process to serve as a type of domain invariant information. In our experiments, we quantitatively and qualitatively demonstrate that the incorporation of edge information is indeed beneficial and effective and enables ELDA to outperform the contemporary state-of-the-art methods on two commonly adopted benchmarks for semantic segmentation based UDA tasks. In addition, we show that ELDA is able to better separate the feature distributions of different classes. We further provide an ablation analysis to justify our design decisions.

==> sections/background.tex <==


% \subsection{Multi-Task Learning}





==> tables/notation.tex <==
\begin{table*}[tp]
\renewcommand{\arraystretch}{1.3}
\newcommand{\mytoprule}{\toprule[1.2pt]}
\centering
\setlength{\tabcolsep}{1.5em}
\footnotesize
\resizebox{.9\linewidth}{!}{%
\begin{tabularx}{\linewidth}{c|l}
\mytoprule
    Symbol & Description  \\
    \mytoprule
    $\Xs$ & A set of training images from the source domain. \\
    $\Xt$ & A set of training images from the target domain. \\
    $\Ys$ & The set of ground truth semantic segmentation labels \\& corresponding to $\Xs$.\\
    \hline
    $\xs$ & An image from the source domain. \\
    $\ys$ & The ground truth semantic segmentation label corresponding to $\xs$. \\
    $\C(\xs)$ & The edges generated by the Canny algorithm from $\xs$. \\
    $\xt$ & An image from the target domain. \\
    $\ypt$ & The pseudo semantic segmentation label corresponding to $\xt$. \\
    $\C(\xt)$ & The edges generated by the Canny algorithm from $\xt$. \\
    \hline
    $\C(\cdot)$ & The Canny operator. \\
    \hline
    $\yshatinit$ & The initial semantic segmentation prediction for $\xs$. \\
    $\ythatinit$ & The initial semantic segmentation prediction for $\xt$. \\
    $\yshatfinal$ & The final semantic segmentation prediction for $\xs$. \\
    $\ythatfinal$ & The final semantic segmentation prediction for $\xt$. \\
    $\eshatinit$ & The initial edge prediction for $\xs$. \\
    $\ethatinit$ & The initial edge prediction for $\xt$. \\
    $\eshatfinal$ & The final edge prediction for $\xs$. \\
    $\ethatfinal$ & The final edge prediction for $\xt$. \\
    $\lambda$ & A balancing factor for the segmentation and edge prediction tasks.\\
    \mytoprule
\end{tabularx}}
\caption{A list of the symbols used in this paper.}
\label{tab:supp:notation}
\end{table*}

==> tables/sigma.tex <==
\begin{table*}[t]
\centering
{\setlength{\tabcolsep}{2em}
\resizebox{.6\textwidth}{!}{%
\renewcommand{\arraystretch}{1.2}
\newcommand{\mytoprule}{\toprule[1.5pt]}
\footnotesize
\begin{tabular}{l|c|c|c}
\hline
\(\sigma\) & 1 & 2 & 3 \\
\hline
mIOU & 53.6 & \textbf{54.0} & 53.7 \\

\mytoprule
\end{tabular}}}
\caption{Ablation study on \(\sigma\).}
\label{tab:sigma}
\end{table*}

==> user-defined/config.tex <==
% default spacing
\setstretch{1.2}

% style of code listing
\lstset{
    % the size of the fonts that are used for the code
    basicstyle=\ttfamily\footnotesize,
    % sets automatic line breaking
    breaklines=true,
    % adds a frame around the code
    frame=single,
    % where to put the line-numbers; possible values are (none, left, right)
    numbers=left,
    % how far the line-numbers are from the code
    numbersep=5pt,
    % the style that is used for the line-numbers
    numberstyle=\scriptsize,
}

% default is centered tabular
\BeforeBeginEnvironment{tabular}{\begin{center}}
\AfterEndEnvironment{tabular}{\end{center}}

% Registering new authors
\FXRegisterAuthor{fon}{afon}{Fiona}


==> user-defined/newcommand.tex <==
\newcommand{\makecover}[1]{
\begin{titlepage}
    \centering
    \vspace*{.75in}
    {\Huge \sc The ELSAToolbox Package}
    
    \vspace*{.25in}
    {\Huge \sc User Manual}
    
    \vspace{.5in}
    {\Large IT Group, ELSA Lab}
    
    \vfill
    \includegraphics[width=.2\linewidth]{%
        images/elsa-logo.png}
    
    Department of Computer Science
    
    National Tsing Hua University
    
    Taiwan
    
    #1
\end{titlepage}
}

\newcommand{\maketoc}{
    \tableofcontents
    \thispagestyle{empty}
    \clearpage
}

\newcommand{\env}[1]{\texttt{#1}}
\newcommand{\pkg}[1]{\texttt{#1}}
\newcommand{\opt}[1]{\texttt{#1}}
\newcommand{\elsatoolbox}{\pkg{elsatoolbox}}


==> user-defined/usepackage.tex <==
\usepackage[top=1in,bottom=1in]{geometry}
\usepackage[nottoc]{tocbibind}
\usepackage{listings}

